Data Incubation -- Synthesizing Missing Data for Handwriting Recognition

In this paper, we demonstrate how a generative model can be used to build a better recognizer through the control of content and style. We are building an online handwriting recognizer from a modest amount of training samples. By training our controllable handwriting synthesizer on the same data, we can synthesize handwriting with previously underrepresented content (e.g., URLs and email addresses) and style (e.g., cursive and slanted). Moreover, we propose a framework to analyze a recognizer that is trained with a mixture of real and synthetic training data. We use the framework to optimize data synthesis and demonstrate significant improvement on handwriting recognition over a model trained on real data only. Overall, we achieve a 66% reduction in Character Error Rate.

==> recipe.tex <==


\section{Synthesize training data}





How do we efficiently utilize generative models to synthesize training data for a downstream recognizer? 
In this section, we propose a systematic framework that identifies beneficial generative settings and underlying issues of the synthetic data. 
Our recipe is motivated by the recent evaluation metric widely used to access the generation quality of a generative adversarial network~\cite{shmelkov2018good}.





The proposed framework is based on Table~\ref{table: wer definition}. 
Given a synthetic dataset (which is randomly split into training, validation, and test sets) of interest, we train three recognizers --- one using only the real training data, one using only the synthetic training data, and the other using both.
Each of the three models are evaluated by Character Error Rates (CERs) using real and synthetic test sets, as denoted in Table~\ref{table: wer definition}. 
Examining these CER values enables us to systematically evaluate the effect of training with the synthetic dataset.


We denote by $\mS_e$ the support of the empirical data distribution (formed by the collected training dataset), by $\mS_s$ the support of the synthetic data distribution, and by $\mS_r$ the support of the real data distribution in-the-wild.
Note that since we have a limited number of collected real data, $\mS_e$ only partially covers $\mS_r$, \eg, it lacks certain content and style.
The following conditions can arise:



\paragraph{Case 1: synthetic data contain exploitable artifacts.}
When the synthetic data contains artifacts that correlate with content, the recognizer trained on the synthetic data can exploit these artifacts, \ie, we have low \WERtrainSS and \WERtestSS.  
However, the same recognizer will perform poorly on real data which lack the exploitable artifacts, \ie, high \WERtestSR.  


\paragraph{Case 2:  $\mS_s \subset \mS_r$.}
In this case, we have a lower diversity in the synthetic data than in the real data, \ie, \WERtestSR > \WERtestRR. 
When the synthetic data only contain typical samples, \ie, data that appear more frequently, we have \WERtestRR > \WERtestRS.
As we have discussed in \secref{sec: models}, when we use a high sampling bias to generate data, the synthetic dataset contains mostly clean and typical handwriting. 
Thus, the recognizer trained on synthetic data will perform poorly on real handwriting, which can be messy sometimes.



\paragraph{Case 3: $\mS_s \supset \mS_e$.}
This is the scenario where the recognizer can benefit from the synthetic data.
By filling in missing content and style, synthetic data increase both the number and the diversity of training data, and thereby improve the performance of downstream recognizers.
In this case, since the synthetic data is more complex than the collected real data, we have \WERtestRS > \WERtestRR and \WERtestSS > \WERtestRR.
Note that we need to pay attention on the style and content that we introduce to $\mS_s$ --- we do not want to overfill the synthetic dataset with words and handwriting styles that rarely appear in the real world.
As discussed before, when we use a small sampling bias to synthesize data, we generate handwriting of a wide variety.
As we will see in the experiments, while it increases the diversity of our training data, it may decrease the performance on real test set.
Using the proposed training procedure, we are able to choose the optimal sampling bias.









\input{table_cer}











==> table_cer.tex <==



\begin{table}[t]
	\caption{Proposed framework to evaluate the effect of synthesized data. Given a synthetic dataset to be evaluate, we train three recognizers, on real data, synthetic data, and both kinds of data. We compute their CERs, denoted below.}
	\label{table: wer definition}
	\small
	\centering
	\setlength{\tabcolsep}{3pt}
	\vspace{-3mm}
	\begin{adjustbox}{max width=\linewidth}
		\begin{tabular}{p{30mm}cccc}
			\toprule
			&
			\makecell{Training CER  \\ on real} &  
			\makecell{Training CER \\ on synthetic} &  
			\makecell{Test CER  \\ on real } &  
			\makecell{Test CER \\ on synthetic} 
			\\   
			\midrule
			Train real & 
			\WERtrainRR & 
			\WERtrainRS &
			\WERtestRR & 
			\WERtestRS
			\\
			Train synthetic & 
			\WERtrainSR & 
			\WERtrainSS & 
			\WERtestSR & 
			\WERtestSS
			\\
			Train real and synthetic & 
			\WERtrainBR & 
			\WERtrainBS & 
			\WERtestBR & 
			\WERtestBS
			\\
			\bottomrule
		\end{tabular}
	\end{adjustbox}
\end{table}



==> table_english.tex <==



\begin{table}[t]
	\caption{CER values for our diagnostics.}
	\label{table: english}
	\small
	\centering
	\def\rowpad{2mm} 
	\setlength{\tabcolsep}{3pt}
	\begin{adjustbox}{max width=\linewidth}
		\begin{tabular}{cccccc}
			\toprule
			\makecell{Generative \\ model  bias}  & 
			\makecell{Training \\ data type} &
			\makecell{Training WER  \\ on real} &  
			\makecell{Training WER \\ on synthetic} &  
			\makecell{Test WER  \\ on real } &  
			\makecell{Test WER \\ on synthetic} 
			\\   
			\midrule
			\multirow{3}{*}{0} & 
			real & 
			$0.76 \pm 0.06$  &  %
			- & %
			$4.93 \pm 0.11$ & %
			$20.9$  %
			\\
			& 
			synthetic &
			- & %
			8.88 & %
			5.27 & %
			12.3 %
			\\
			& 
			real + synthetic & 
			- &  %
			- &  %
			4.02 &  %
			11.8  %
			\\[\rowpad]
			\multirow{3}{*}{0.05} & 
			real & 
			$0.76 \pm 0.06$  &  %
			- & %
			$4.93 \pm 0.11$ & %
			$17.1$  %
			\\
			& 
			synthetic &
			- & %
			5.55 & %
			5.09 & %
			9.01 %
			\\
			& 
			real + synthetic & 
			- &  %
			- &  %
			4.0 &  %
			8.8  %
			\\[\rowpad]
			\multirow{3}{*}{0.1} & 
			real & 
			$0.76 \pm 0.06$  &  %
			- & %
			$4.93 \pm 0.11$ & %
			$14.2$  %
			\\
			& 
			synthetic &
			- & %
			4.01 & %
			5.26 & %
			7.05 %
			\\
			& 
			real + synthetic & 
			- &  %
			- &  %
			4.03 &  %
			6.9  %
			\\[\rowpad]
			\multirow{3}{*}{0.2} & 
			real & 
			$0.76 \pm 0.06$  &  %
			- & %
			$4.93 \pm 0.11$ & %
			$10.5$  %
			\\
			& 
			synthetic &
			- & %
			2.35 & %
			5.9 & %
			4.98 %
			\\
			& 
			real + synthetic & 
			- &  %
			- &  %
			4.23 &  %
			4.67  %
			\\[\rowpad]
			\multirow{3}{*}{0.25} & 
			real & 
			$0.76 \pm 0.06$  &  %
			- & %
			$4.93 \pm 0.11$ & %
			$9.62$  %
			\\
			& 
			synthetic &
			- & %
			1.81 & %
			6.12 & %
			4.24 %
			\\
			& 
			real + synthetic & 
			- &  %
			- &  %
			4.26 &  %
			4.22  %
			\\[\rowpad]
			\multirow{3}{*}{0.35} & 
			real & 
			$0.76 \pm 0.06$  &  %
			- & %
			$4.93 \pm 0.11$ & %
			$8.13$  %
			\\
			& 
			synthetic &
			- & %
			1.21 & %
			6.56 & %
			3.26 %
			\\
			& 
			real + synthetic & 
			- &  %
			- &  %
			4.28 &  %
			3.20  %
			\\[\rowpad]
			\multirow{3}{*}{0.5} & 
			real & 
			$0.76 \pm 0.06$  &  %
			- & %
			$4.93 \pm 0.11$ & %
			$6.76$  %
			\\
			& 
			synthetic &
			- & %
			0.89 & %
			7.65 & %
			2.57 %
			\\
			& 
			real + synthetic & 
			- &  %
			- &  %
			4.43 &  %
			2.4  %
			\\%[\rowpad]
			\bottomrule
		\end{tabular}
	\end{adjustbox}
\end{table}






\begin{table}[t]
	\caption{
		CER values for our diagnostics.  1M synthetic data. \\
		\WERtrainRR  = $0.76 \pm 0.06$,   
		\WERtestRR = $4.93 \pm 0.11$  
	}
	\label{table: english}
	\small
	\centering
	\def\rowpad{2mm} 
	\setlength{\tabcolsep}{3pt}
	\begin{adjustbox}{max width=\linewidth}
		\begin{tabular}{lrrrrr}
			\toprule
			& %
			\makecell{\WERtestRS} &  
			\makecell{\WERtrainSS} &  
			\makecell{\WERtestSR} & 
			\makecell{\WERtestSS} & 
			\makecell{\WERtestBR} 
			\\   
			\midrule
			bias = 0 & %
			20.9 & %
			8.88 & %
			5.27 & %
			12.3 & %
			4.02 %
			\\
			bias = 0.05 & %
			17.1 & %
			5.55 & %
			5.09 & %
			9.01 & %
			4.00 %
			\\
			bias = 0.1 & %
			14.2 & %
			4.01 & %
			5.26 & %
			7.05 & %
			4.03 %
			\\
			bias = 0.2 & %
			10.5 & %
			2.35 & %
			5.90 & %
			4.98 & %
			4.23 %
			\\
			bias = 0.25 & %
			9.62 & %
			1.81 & %
			6.12 & %
			4.24 & %
			4.26 %
			\\
			bias = 0.35 & %
			8.13 & %
			1.21 & %
			6.56 & %
			3.26 & %
			4.28 %
			\\
			bias = 0.5 & %
			6.76 & %
			0.89 & %
			7.65 & %
			2.57 & %
			4.43 %
			\\
			\bottomrule
		\end{tabular}
	\end{adjustbox}
\end{table}






==> table_final.tex <==


\begin{table}[t]
	\caption{
		CER of our English and multilingual recognizers.  The recognizers in the first three columns share the same corpus (the corpus of the collected EN (or multilingual) data, ori.~corpus), and they demonstrate the effect of filling in missing style.  The last column demonstrates the effect of filling in both content and style --- we expand the synthesis corpus by a large multilingual corpus and other under-represented content in ori.~corpus.
		We evaluate the EN recognizers on the collected English Test set (EN Test).
		We evaluate the multilingual recognizers on two datasets --- the collected test set (Test) and a separate test set that contains special patterns like URLs, street names, and fake Email addresses (SP).  
	}
	\label{table: final}
	\small
	\centering
	\def\rowpad{2mm} 
	\setlength{\tabcolsep}{3.6pt}
	\vspace{-2mm}
	\begin{adjustbox}{max width=\linewidth}
		\begin{tabular}{lcccc}
			\toprule
			\makecell[l]{training data}& 
			\makecell{real-only \\ (ori. corpus)} &  
			\makecell{synthetic-only \\ (ori. corpus)} &
			\makecell{real + synthetic \\ (ori. corpus)} &  
			\makecell{real + synthetic \\ (expanded corpus)} 
			\\   
			\midrule
			\# EN training data (M)& 
			0.3 &  %
			4.0  & %
			4.3  \hspace{0.5mm}  $(0.3 + 4)$ & %
			-
			\\
			CER on EN Test (\%)& 
			4.94 &  %
			4.17  \hspace{0.2mm} $(\downarrow 16 \,\%)$ & %
			3.56 \hspace{0.2mm}$(\downarrow 28 \,\%)$ & %
			- %
			\\
			\midrule
			\# training data (M)& 
			0.6 &  %
			3.0  & %
			3.6  \hspace{0.2mm}  $(0.6 + 3)$ & %
			\textbf{8.1  \hspace{0.2mm} $(0.6 + 7.5)$}  %
			\\
			CER on Test (\%)& 
			8.22 &  %
			5.16 \hspace{0.2mm} $(\downarrow 37 \,\%)$ & %
			4.46 \hspace{0.2mm}$(\downarrow 46 \,\%)$ & %
			\textbf{2.77  \hspace{0.2mm} $(\downarrow \mathbf{66 \,	\%})$}  %
			\\
			\makecell[l]{CER on SP (\%)} & 
			18.5 &  %
			18.9 \hspace{0.2mm} $(\uparrow 2 \,\%)$ & %
			16.9 \hspace{0.2mm}$(\downarrow 9 \,\%)$ & %
			\textbf{6.28  \hspace{0.2mm} $(\downarrow \mathbf{66 \,	\%})$}  %
			\\
			\bottomrule
		\end{tabular}
	\end{adjustbox}
\end{table}







==> table_symptom.tex <==
diggdi

\begin{table}[t]
	\caption{Generative model diagnostic table}
	\label{table: diagnostic}
	\small
	\centering
	\def\rowpad{2mm} 
	\def\tworowpad{6mm} 
	\setlength{\tabcolsep}{6pt}
	\begin{adjustbox}{max width=\linewidth}
		\begin{tabular}{p{25mm}l}
			\toprule
			\multicolumn{1}{c}{Problem} &
			\multicolumn{1}{c}{Symptoms}
			\\   
			\midrule
			domain shift &
			\WERtestRS $\gg$ \WERtestRR
			\\[\rowpad]
			samples too easy &
			\makecell[tl]{\WERtrainRR $\gg$ \WERtrainRS,  \WERtestSR $\gg$ \WERtestRR } %
			\\[\rowpad]
			low-quality output &
			\makecell[tl]{\WERtrainSS $\gg$ \WERtrainRR, \WERtestSS $\gg$ \WERtestRR, \\ \WERtestRS $\gg$ \WERtestRR }
			\\[\tworowpad]
			exploitable artifacts &
			\makecell[tl]{small \WERtrainSS but high \WERtestSR, small \WERtestSS }
			\\
			\bottomrule
		\end{tabular}
	\end{adjustbox}
\end{table}


